Monolayer and bilayer PtCl$_3$: Energetics, magnetism, and band topology

Two-dimensional (2D) magnetic materials hosting nontrivial topological states are interesting for fundamental research as well as practical applications. Recently, the topological state of 2D Weyl half-semimetal (WHS) was proposed, which hosts fully spin polarized Weyl points robust against spin-orbit coupling in a 2D ferromagnetic system, and single-layer PtCl$_3$ was predicted as a platform for realizing this state. Here, we perform an extensive search of 2D PtCl$_3$ structures, by using the particle swarm optimization technique and density functional theory calculation. We show that the desired PtCl$_3$ phase corresponds to the most stable one at its stoichiometry. The 2D structure also possesses good thermal stability up to 600 K. We suggest SnS$_2$ as a substrate for the growth of 2D PtCl$_3$, which has excellent lattice matching and preserves the WHS state in PtCl$_3$. We find that uniaxial strains along the zigzag direction maintain the WHS state, whereas small strains along the armchair direction drives a topological phase transition from the WHS to a quantum anomalous Hall (QAH) insulator phase. Furthermore, we study bilayer PtCl$_3$ and show that the stacking configuration has strong impact on the magnetism and the electronic band structure. Particularly, the $AA'$ stacked bilayer PtCl$_3$ realizes an interesting topological state -- the 2D antiferromagnetic mirror Chern insulator, which has a pair of topological gapless edge bands. Our work provides guidance for the experimental realization of 2D PtCl$_3$ and will facilitate the study of 2D magnetic topological states, including WHS, QAH insulator, and magnetic mirror Chern insulator states.

==> Makefile <==
LATEX = latex 
BIBTEX = bibtex
DVIPDF = dvipdfmx
PDFLATEX = pdflatex


tex_base =PtCl3v220315

pdf: 
	$(PDFLATEX)  $(tex_base)	
	$(BIBTEX)    $(tex_base)
	$(PDFLATEX)  $(tex_base)	
	$(PDFLATEX)  $(tex_base)	

clean :
	rm -vf $(tex_base).dvi $(tex_base).log $(tex_base).aux $(tex_base).bbl \
	$(tex_base).blg *$(tex_base).ilg $(tex_base).toc $(tex_base).lof \
	$(tex_base).lot $(tex_base).idx $(tex_base).ind $(tex_base).out \
	$(tex_base).ps figs/*.pdf



